Domains for Higher-Order Games

We study two-player inclusion games played over word-generating higher-order recursion schemes. While inclusion checks are known to capture verification problems, two-player games generalize this relationship to program synthesis. In such games, non-terminals of the grammar are controlled by opposing players. The goal of the existential player is to avoid producing a word that lies outside of a regular language of safe words. We contribute a new domain that provides a representation of the winning region of such games. Our domain is based on (functions over) potentially infinite Boolean formulas with words as atomic propositions. We develop an abstract interpretation framework that we instantiate to abstract this domain into a domain where the propositions are replaced by states of a finite automaton. This second domain is therefore finite and we obtain, via standard fixed-point techniques, a direct algorithm for the analysis of two-player inclusion games. We show, via a second instantiation of the framework, that our finite domain can be optimized, leading to a (k+1)EXP algorithm for order-k recursion schemes. We give a matching lower bound, showing that our approach is optimal. Since our approach is based on standard Kleene iteration, existing techniques and tools for fixed-point computations can be applied.

==> content/semantics.tex <==
\section{Semantics}



==> style/abbrev_de.tex <==
% ######################
% ABBREVIATIONS
% ######################

% small
\newcommand{\bzgl}
{bzgl.~}

\newcommand{\obda}
{o.B.d.A.~}

\newcommand{\bzw}
{bzw.~}

% capital
\newcommand{\Obda}
{O.B.d.A.~}


==> style/abbrev_en.tex <==
% ######################
% ABBREVIATIONS
% ######################

% small
\newcommand{\wrt}
{wrt.~}

\newcommand{\ie}
{i.e.~}

\newcommand{\eg}
{e.g.~}

\newcommand{\resp}
{resp.~}

\newcommand{\sth}
{s.t.~}

\newcommand{\wolog}
{wlog.~}

% capital
\newcommand{\Ie}
{I.e.~}

\newcommand{\Eg}
{E.g.~}

\newcommand{\Wolog}
{Wlog.~}


==> style/algo.tex <==
% ############
% ALGORITHMS
% ############

% algorithms
\usepackage{algorithmicx}
\usepackage{algpseudocode}

% code for "indentation guide"-style verticle lines
\makeatletter
\def\therule{\makebox[\algorithmicindent][l]{\hspace*{.5em}\vrule height .75\baselineskip depth .25\baselineskip}}%

\newtoks\therules% Contains rules
\therules={}% Start with empty token list
\def\appendto#1#2{\expandafter#1\expandafter{\the#1#2}}% Append to token list
\def\gobblefirst#1{% Remove (first) from token list
  #1\expandafter\expandafter\expandafter{\expandafter\@gobble\the#1}}%

\let\oldState\State
\def\LState{\oldState\unskip\the\therules}% New line-state
\let\State\LState
\let\Cmd\LState

\def\pushindent{\appendto\therules\therule}%
\def\popindent{\gobblefirst\therules}%
\def\printindent{\unskip\the\therules}%
\def\printandpush{\printindent\pushindent}%
\def\popandprint{\popindent\printindent}%

\algdef{SE}[WHILE]{While}{EndWhile}[1]
  {\printandpush\algorithmicwhile\ #1\ \algorithmicdo}
  {\popandprint\algorithmicend\ \algorithmicwhile}%
\algdef{SE}[FOR]{For}{EndFor}[1]
  {\printandpush\algorithmicfor\ #1\ \algorithmicdo}
  {\popandprint\algorithmicend\ \algorithmicfor}%
\algdef{S}[FOR]{ForAll}[1]
  {\printindent\algorithmicforall\ #1\ \algorithmicdo}%
\algdef{SE}[LOOP]{Loop}{EndLoop}
  {\printandpush\algorithmicloop}
  {\popandprint\algorithmicend\ \algorithmicloop}%
\algdef{SE}[REPEAT]{Repeat}{Until}
  {\printandpush\algorithmicrepeat}[1]
  {\popandprint\algorithmicuntil\ #1}%
\algdef{SE}[IF]{If}{EndIf}[1]
  {\printandpush\algorithmicif\ #1\ \algorithmicthen}
  {\popandprint\algorithmicend\ \algorithmicif}%
\algdef{C}[IF]{IF}{ElsIf}[1]
  {\popandprint\pushindent\algorithmicelse\ \algorithmicif\ #1\ \algorithmicthen}%
\algdef{Ce}[ELSE]{IF}{Else}{EndIf}
  {\popandprint\pushindent\algorithmicelse}%
\algdef{SE}[PROCEDURE]{Procedure}{EndProcedure}[2]
   {\printandpush\algorithmicprocedure\ \textproc{#1}\ifthenelse{\equal{#2}{}}{}{(#2)}}%
   {\popandprint\algorithmicend\ \algorithmicprocedure}%
\algdef{SE}[FUNCTION]{Function}{EndFunction}[2]
   {\printandpush\algorithmicfunction\ \textproc{#1}\ifthenelse{\equal{#2}{}}{}{(#2)}}%
   {\popandprint\algorithmicend\ \algorithmicfunction}%
\makeatother

% C-style comments
\renewcommand {\algorithmiccomment}[1]
    {\hfill $/ \!/$ #1}
   
% return on new line
\let\oldReturn\Return
\renewcommand{\Return}{\LState\oldReturn}

% commands like in algorith2e
\newcommand {\ForLoop} [2]
{
    \For {#1}
        #2
    \EndFor
}

\newcommand {\WhileLoop} [2]
{
    \While {#1}
        #2
    \EndWhile
}

\newcommand {\IfCond} [2]
{
    \If {#1}
        #2
    \EndIf
}

\newcommand {\IfElseCond} [3]
{
    \If {#1}
        #2
    \Else
        #3
    \EndIf
}


==> style/article.tex <==
% ########################
% ARTICLE SPECIFIC STUFF
% ########################

% Festlegung Art der Zitierung - Havardmethode: Abkuerzung Autor + Jahr
\usepackage[style=alphabetic,maxbibnames=9,maxcitenames=9,backend=bibtex,]{biblatex}

% underlining
\usepackage{ulem}

% spacing between lines of text
\usepackage{setspace}

% enumerate etc
\usepackage{paralist}

% keyword index
\usepackage{makeidx}

% create keyword index
\makeindex

%% abbreviation index
%\usepackage[german]{nomencl}
%\let\abbrev\nomenclature

% border size
\usepackage{geometry}
\geometry{left=2.5cm, right=2.5cm, top=2.5cm, bottom=2cm, foot=1cm}

% Indentation
% space between lines
\onehalfspacing
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000

% references
\PassOptionsToPackage{obeyspaces}{url}
\usepackage[bookmarksnumbered]{hyperref} 

% line break in URLs
%\usepackage[hyphens,obeyspaces,spaces]{url}

\makeatletter
\g@addto@macro{\UrlBreaks}{\UrlOrds}
\makeatother

% newline after paragraph, paragraph bold and underlined
\makeatletter
\renewcommand {\paragraph}
{
    \@startsection
        {paragraph} % name
        {4}         % level
        {\z@}       % indent     
        {0ex \@plus -1ex \@minus -.2ex} % beforeskip
        %{-3.25ex\@plus -1ex \@minus -.2ex} % beforeskip
        {0.01ex \@plus .2ex}                % afterskip
        %{1.5ex \@plus -2ex}                % afterskip
        {\normalfont\normalsize\bfseries} % style of heading
}
\makeatother

% proof in bold font, colon and newline afterwards
\makeatletter
\renewenvironment{proof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\\*\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother

% proof in bold font, colon and newline afterwards
\makeatletter
\newenvironment{shortproof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother

% set emph back to normal (instead of underlined)
\normalem 

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother

% Theorem numbering
\def\theoremnumberstyle{changesection}

% Theoremstyle
\newtheoremstyle{withnumber} % name
{0.4cm}                    % Space above
{0.6cm}                    % Space below
{\normalfont}                   % Body font
{}                           % Indent amount
{\bfseries}                   % Theorem head font
{\newline}                          % Punctuation after theorem head
{0.2cm}                       % Space after theorem head
{#2 #1\thmnote{: \ #3}}  % Theorem head spec (can be left empty, meaning ‘normal’)

\newtheoremstyle{nonumber} % name
{0.4cm}                    % Space above
{0.6cm}                    % Space below
{\normalfont}                   % Body font
{}                           % Indent amount
{\bfseries}                   % Theorem head font
{\newline}                          % Punctuation after theorem head
{0.2cm}                       % Space after theorem head
{#1\thmnote{: \ #3}}  % Theorem head spec (can be left empty, meaning ‘normal’)

\theoremstyle{withnumber} 

% itemize/enumerate at the beginning of a thm
\newenvironment{thmenumerate}
{
    \leavevmode\vspace{-2.2em}
    \begin{enumerate}
    }
    {
    \end{enumerate}
}

\newenvironment{thmitemize}
{
    \leavevmode\vspace{-2.2em}
    \begin{itemize}
    }
    {
    \end{itemize}
}

% chapters = sections (otherwise numbering will not work)
\let\chapter\section

% subsections numbered by capital arabic letters
%\renewcommand{\thesubsection}{\thesection.\Roman{subsection}}
\renewcommand{\thesubsection}{\Alph{subsection})}

\usepackage{secdot}
\sectionpunct{subsection}{ }

% captions
\usepackage{capt-of}
\usepackage{caption}
\DeclareCaptionFont{white}{\color{white}}
%\DeclareCaptionFormat{listing}
%{
%    \colorbox[cmyk]{1, 1, 1,0.01}
%    {
%        \parbox{\textwidth}
%        {\hspace{15pt}#1#2#3}
%    }
%}
%\captionsetup[lstlisting]
%{
%    format=listing,
%    labelfont=white,
%    textfont=white,
%    singlelinecheck=false,
%    margin=0pt,
%    font={bf,footnotesize}
%}

% listings
\usepackage{listings}
\lstset{
    numbers=left,
    numberstyle=\tiny,
    numbersep=5pt,
    keywordstyle=\color{black}\bfseries,
    stringstyle=\ttfamily,
    showstringspaces=false,
    basicstyle=\footnotesize,
    captionpos=b
}
\lstset{language=java}
% Listings
\lstset{
    basicstyle=\fontsize{9}{9}\ttfamily, % Standardschrift
    numbers=left,               % Ort der Zeilennummern
    numberstyle=\tiny,          % Stil der Zeilennummern
    %stepnumber=2,               % Abstand zwischen den Zeilennummern
    numbersep=5pt,              % Abstand der Nummern zum Text
    tabsize=4,                  % Groesse von Tabs
    extendedchars=true,         %
    breaklines=true,            % Zeilen werden Umgebrochen
    keywordstyle=\text,
    %frame=b,         
    stringstyle=\color{black}\ttfamily, % Farbe der String
    showspaces=false,           % Leerzeichen anzeigen ?
    showtabs=false,             % Tabs anzeigen ?
    xleftmargin=5pt,
    framexleftmargin=17pt,
    framexrightmargin=5pt,
    framexbottommargin=4pt,
    %backgroundcolor=\color{lightgray},
    showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
    captionpos=t,     
}

\lstloadlanguages{% Check Dokumentation for further languages ...
    %[Visual]Basic
    %Pascal
    %C
    %C++
    %XML
    %HTML
    Java
}

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}

\usepackage[headsepline]{scrlayer-scrpage}
%\clearpairofpagestyles
\clearscrheadfoot
\ihead{\normalfont \headmark}
\cfoot{\Large \pagemark}
\automark[]{section}

\makeatletter
\newcommand {\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand {\problemshort}[1]{\gdef\@problemshort{#1}}% Store problem short notation
\newcommand {\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand {\problemparameter}[1]{\gdef\@problemparameter{#1}}% Store problem parameter
\newcommand {\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question

\NewEnviron{problem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
%    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocDecide:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\NewEnviron{compproblem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocCompute:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\makeatother

% don't show subsections in TOC
\setcounter{tocdepth}{1}


==> style/commands.tex <==
% ##########
% COMMANDS
% ##########

% custom emph
\newcommand {\emphbf}[1]
{ \emph{#1} }

% bold + italic
\newcommand {\textbfit} [1]
{ \textbf{\textit{#1}} }

% monospace (+ bold & italic)
\newcommand {\mono} [1]
{ \texttt {#1} }

\newcommand {\monobf} [1]
{ \texttt {\bfseries #1} }

\newcommand {\monobfit} [1]
{ \texttt {\bfseries \itshape #1} }

\newcommand {\monoit} [1]
{ \texttt {\itshape #1} }

% fake capital greek letters
%\newcommand {\Alpha} {A}
%\newcommand {\Beta} {B}
%\newcommand {\Epsilon} {E}
%\newcommand {\Zeta} {Z}
%\newcommand {\Eta} {H}
%\newcommand {\Iota} {I}
%\newcommand {\Kappa} {K}
%\newcommand {\Mu} {M}
%\newcommand {\Tau} {T}
%\newcommand {\Chi} {X}

% blackboard bold letters
\newcommand {\A} {{\mathbb A}}
\providecommand\B{}
\renewcommand {\B} {{\mathbb B}}
\providecommand{\C}{}
\renewcommand {\C} {{\mathbb C}}
\newcommand {\D} {{\mathbb D}}
\newcommand {\E} {{\mathbb E}}
\newcommand {\F} {{\mathbb F}}
\providecommand {\G} {}
\renewcommand {\G} {{\mathbb G}}
\renewcommand {\H} {{\mathbb H}}
\newcommand {\I} {{\mathbb I}}
\newcommand {\J} {{\mathbb J}}
\newcommand {\K} {{\mathbb K}}
\renewcommand {\L} {{\mathbb L}}
\providecommand {\M} {}
\renewcommand {\M} {{\mathbb M}}
\newcommand {\N} {{\mathbb N}}
\renewcommand {\O} {{\mathbb O}}
\renewcommand {\P} {{\mathbb P}}
\newcommand {\Q} {{\mathbb Q}}
\newcommand {\R} {{\mathbb R}}
\renewcommand {\S} {{\mathbb S}}
\providecommand {\T} {}
\renewcommand {\T} {{\mathbb T}}
\providecommand{\U}{}
\renewcommand {\U} {{\mathbb U}}
\newcommand {\V} {{\mathbb V}}
\newcommand {\W} {{\mathbb W}}
\newcommand {\X} {{\mathbb X}}
\newcommand {\Y} {{\mathbb Y}}
\newcommand {\Z} {{\mathbb Z}}

% caligraphic letters
\newcommand {\calA} {\mathcal{A}}
\newcommand {\calB} {\mathcal{B}}
\newcommand {\calC} {\mathcal{C}}
\newcommand {\calD} {\mathcal{D}}
\newcommand {\calE} {\mathcal{E}}
\newcommand {\calF} {\mathcal{F}}
\newcommand {\calG} {\mathcal{G}}
\newcommand {\calH} {\mathcal{H}}
\newcommand {\calI} {\mathcal{I}}
\newcommand {\calJ} {\mathcal{J}}
\newcommand {\calK} {\mathcal{K}}
\newcommand {\calL} {\mathcal{L}}
\newcommand {\calM} {\mathcal{M}}
\newcommand {\calN} {\mathcal{N}}
\newcommand {\calO} {\mathcal{O}}
\newcommand {\calP} {\mathcal{P}}
\newcommand {\calQ} {\mathcal{Q}}
\newcommand {\calR} {\mathcal{R}}
\newcommand {\calS} {\mathcal{S}}
\newcommand {\calT} {\mathcal{T}}
\newcommand {\calU} {\mathcal{U}}
\newcommand {\calV} {\mathcal{V}}
\newcommand {\calW} {\mathcal{W}}
\newcommand {\calX} {\mathcal{X}}
\newcommand {\calY} {\mathcal{Y}}
\newcommand {\calZ} {\mathcal{Z}}


==> style/definitions.tex <==
% ##################
% DEFINITIONS
% ##################

%
% Basic stuff
%

\newcommand { \from }
{ \leftarrow }

\newcommand {\Rplus} 
{ \R_{>0} }

\newcommand {\true}
{\mathit{true}}

\newcommand {\false}
{\mathit{false}}

\newcommand {\monotrue}
{\mathit{true}}

\newcommand {\monofalse}
{\mathit{false}}

\newcommand { \ifalse }
{ \mathit{false} }

\newcommand { \itrue }
{ \mathit{true} }

\newcommand {\oneto} [1]
{\left\{ 1, \ldots, #1\right\}}

\newcommand {\zeroto} [1]
{\left\{ 0, \ldots, #1\right\}}

\newcommand {\arity} [1]
{ {\scriptstyle / #1 } }

% small @
\newcommand {\at}
{
    \raisebox{0.5mm}{\scalebox{0.7}[0.7]{@}}
}

% corresponds to
\newcommand\corrto{%
    \let\savearraystretch\arraystretch
    \renewcommand\arraystretch{0.3}
    \begin{array}{c}
        \stretchto{
            \scalerel*[\widthof{=}]{\wedge}
            {\rule{1ex}{3ex}}%
        }{0.5ex}\\ 
        =%
    \end{array}
    \let\arraystretch\savearraystretch
}

% stacked logical operators
\newcommand{\wedgevee}
{
    \mathrel{\substack{\wedge\\\vee}}
}
\newcommand{\veewedge}
{
    \mathrel{\substack{\vee\\\wedge}}
}

\newcommand{\poly}
{\mathrm{poly}}

% small mid for (E)BNF
\newcommand{\bnf}
{\:\shortmid\:}

%
% Sets
%

\newcommand{\card}[1]
{\left|#1\right|}

\newcommand {\set} [1]
{ \left\{ #1 \right\} }

\newcommand {\Set} [2]
{ \left\{ #1 \ \middle| \ #2 \right\} }

\newcommand {\smallset} [2]
{ \{ #1 \mid #2 \} }

\newcommand {\ideal} [1]
{ \langle \ #1 \ \rangle}

\newcommand {\Ideal} [2]
{ \langle \ #1 \mid #2 \ \rangle}

\newcommand {\pwrset} [1]
{ {\mathcal P} \left( #1 \right)}

%
% Set operations
%

\newcommand* {\medcap}
{ \mathbin{\scalebox{1.5}{\ensuremath{\cup}}} }
\newcommand* {\medcup}
{ \mathop{\mathbin{\scalebox{1.5}{\ensuremath{\cup}}}} } 
\newcommand* {\hugecup}
{ \mathop{\mathbin{\scalebox{3}{\ensuremath{\cup}}}} }

\newcommand {\bigdotcup}
{\ensuremath{\mathop{\mathaccent\cdot{\bigcup}}}}
\newcommand {\dotcup}
{\ensuremath{\mathop{\mathaccent\cdot\cup}}}

% disjoint union
\makeatletter
\providecommand*{\bigcupdot}{%
    \mathbin{%
        \mathpalette\@bigcupdot{}%
    }%
}
\newcommand*{\@bigcupdot}[2]{%
    \ooalign{%
        $\m@th#1\bigcup$\cr
        \hidewidth$\m@th#1\cdot$\hidewidth
    }%
}
\makeatother

\makeatletter
\providecommand*{\cupdot}{%
    \mathbin{%
        \mathpalette\@cupdot{}%
    }%
}
\newcommand*{\@cupdot}[2]{%
    \ooalign{%
        $\m@th#1\cup$\cr
        \hidewidth$\m@th#1\cdot$\hidewidth
    }%
}
\makeatother

%
% Closures
%

\newcommand{\up}
{\!\uparrow}

\newcommand{\down}
{\!\downarrow}

\newcommand{\dc}[1]
{#1\!\downarrow\ }

\newcommand{\uc}[1]
{#1\!\uparrow\ }

%
% Logic
%

\DeclareDocumentCommand \FO { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \mathsf{FO} }
    { \mathsf{FO} \left( #1 \right) }
}

\newcommand {\sem}[1]
{	\left\llbracket #1 \right\rrbracket }

% inverse models
\makeatletter
\providecommand*{\Dashv}{%
    \mathrel{%
        \mathpalette\@Dashv\vDash
    }%
}
\makeatother

% logical equivalence (\models \ismod)
\newcommand{\lequiv}{\vDash\hspace{-2pt}\Dashv}

%
% Complexity & Turing machines
%

\newcommand {\bigO} [1]
{ \calO \left( {#1} \right) }

\newcommand {\smallO} [1]
{ o \left( #1 \right) }

\newcommand {\bigOmega} [1]
{ \Omega \left( #1 \right) }

\newcommand {\smallOmega} [1]
{ \omega \left( #1 \right) }

\newcommand {\bigTheta} [1]
{ \Theta \left( #1 \right) }

% blank symbol
\newsavebox{\blankbox}
\savebox{\blankbox}{\texttt{aa}}
\newcommand\vartextvisiblespace[1][0.8\wd\blankbox]{%
    \makebox[#1]{\kern.1em\rule{.4pt}{.5ex}%
        \hrulefill%
        \rule{.4pt}{.5ex}\kern.1em}%
}
\newcommand{\blank}{\vartextvisiblespace}% For ease-of-use

\newcommand{\qinit}{q_0}
\newcommand{\qaccept}{q_{\mathit{acc}}}
\newcommand{\qhalt}{q_{\mathit{halt}}}
\newcommand{\qreject}{q_{\mathit{rej}}}

\newcommand {\LOGSPACE}
{\mathsf{L}}
\newcommand {\NLOGSPACE}
{\mathsf{NL}}
\newcommand {\PTIME}
{\mathsf{P}}
\newcommand {\NPTIME}
{\mathsf{NP}}
\newcommand {\PSPACE}
{\mathsf{PSPACE}}
\newcommand {\EXPTIME}
{\mathsf{EXP}}
\newcommand {\EXPSPACE}
{\mathsf{EXPSPACE}}

%
% Words
%

\newcommand{\prefix}[1]
{\text{prefix}(#1)}

\newcommand {\subword}
{\!\preceq}

%
% Automata theory
%

\newcommand {\tow} [1]
{ \xrightarrow{#1}{\to} }

\newcommand{\towi}[2]
{\tow{#1}_{#2}}

\DeclareDocumentCommand \lang { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \calL }
    { \calL \left( #1 \right) }
}
\newcommand {\langm}
{ \calM }
\DeclareDocumentCommand \olang { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \calL^\omega }
    { \calL^\omega \!\left( #1 \right) }
}

\DeclareDocumentCommand \Parikh { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \Psi }
    { \Psi \left( #1 \right) }
}

%
% Grammars
%

% derivation
\newcommand{\derive}{\Rightarrow}
\newcommand{\leftderive}{\derive}

%
% Systems of equations / equalities
%

\newcommand {\tbox} [1]
{ \rho_{#1} }
\newcommand {\var} [1]
{ \Delta_{#1} }
\newcommand {\sol} [1]
{ \sigma_{#1} }

%
% Games
%

\newcommand{\owner}{\mathit{owner}}

\usepackage{ wasysym }

\newcommand {\refuter} { { \fullmoon } }
\newcommand {\prover} { \square }

\newcommand {\players} { \set{\prover, \refuter}}

\newcommand\openbigstar[1][0.7]
{
    {
        \scalerel*{%
        \stackinset{c}{-.125pt}{c}{}{\scalebox{#1}{\color{white}{$\bigstar$}}}
        {%
            $\bigstar$}%
        }
        {\bigstar}
    }
}
\newcommand {\player} { {\openbigstar} }
\newcommand {\opponent} { {\overline{\openbigstar}} }

\newcommand{\last}[1]{#1_{\mathit{last}}}

\newcommand{\Plays}{\mathit{Plays}}
\newcommand{\PlaysFin}{\Plays_{\mathit{fin}}}
\newcommand{\PlaysInf}{\Plays_{\mathit{inf}}}
\newcommand{\PlaysMax}{\Plays_{\mathit{max}}}
\newcommand{\PlaysLive}{\Plays_{\mathit{live}}}
\newcommand{\PlaysDead}{\Plays_{\mathit{dead}}}
\newcommand{\PlaysRefuter}{\Plays_{\refuter}}
\newcommand{\PlaysProver}{\Plays_{\prover}}
\newcommand{\PlaysPlayer}{\Plays_{\player}}
\newcommand{\PlaysOpponent}{\Plays_{\opponent}}

\newcommand{\winningcond}{\mathit{win}}

\newcommand{\Inf}[1]{\text{Inf}\left(#1\right)}

\DeclareDocumentCommand \Attr { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \text{Attr} }
    { \text{Attr} \left( #1 \right) }
}

\DeclareDocumentCommand \CPre { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \text{CPre} }
    { \text{CPre} \left( #1 \right) }
}

%
% Special
%

\newcommand{\Buechi}{B\"uchi}


==> style/exam.tex <==
% ########################
% EXAM SPECIFIC STUFF
% ########################

% Festlegung Art der Zitierung - Havardmethode: Abkuerzung Autor + Jahr
\usepackage[style=alphabetic,backend=bibtex]{biblatex}

% underlining
\usepackage{ulem}

% spacing between lines of text
\usepackage{setspace}

% enumerate etc
\usepackage{paralist}

% keyword index
\usepackage{makeidx}

% create keyword index
\makeindex

%% abbreviation index
%\usepackage[german]{nomencl}
%\let\abbrev\nomenclature

% border size
\usepackage{geometry}
\geometry{left=2.5cm, right=2.5cm, top=2cm, bottom=2cm, foot= 1cm}

% Indentation
% space between lines
\onehalfspacing
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000

% references
\usepackage[bookmarksnumbered]{hyperref} 

% line break in URLs
%\usepackage[hyphens,obeyspaces,spaces]{url}

% newline after paragraph, paragraph bold and underlined
\makeatletter
\renewcommand {\paragraph}
{
    \@startsection
        {paragraph} % name
        {4}         % level
        {\z@}       % indent     
        {0ex \@plus -1ex \@minus -.2ex} % beforeskip
        %{-3.25ex\@plus -1ex \@minus -.2ex} % beforeskip
        {0.01ex \@plus .2ex}                % afterskip
        %{1.5ex \@plus -2ex}                % afterskip
        {\normalfont\normalsize\bfseries\underbar} % style of heading
}
\makeatother

% proof in bold font, colon and newline afterwards
\makeatletter
\renewenvironment{proof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\\*\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother

% set emph back to normal (instead of underlined)
\normalem 

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother

% Theorem numbering
\def\theoremnumberstyle{changesection}

% Bei Nummerierung vom Typ swapped soll abweichend vom Standard
% "5.12. Satz" erscheinen als "5.12 Satz", das heisst ohne
% zusaetzlichen Punkt.
\makeatletter
\def\swappedhead#1#2#3{%
    \thmnumber{#2}\thmname{ #1}%
    \thmnote{ {\the\thm@notefont(#3)}}}
\makeatother

% Theoremstyle
\newtheoremstyle{varthm-roman-break} % name
{0.4cm}                          % Space above
{0.6cm}                          % Space below
{\normalfont}                    % Body font
{}                               % Indent amount
{\bfseries\sffamily}             % Theorem head font
{\newline}                       % Punctuation after theorem head
{0.2cm}                          % Space after theorem head
{\thmnote{#3}}                   % Theorem head spec


\swapnumbers
\theoremstyle{varthm-roman-break} 

% itemize/enumerate at the beginning of a thm
\newenvironment{thmenumerate}
{
    \leavevmode\vspace{-1.4em}
    \begin{enumerate}
    }
    {
    \end{enumerate}
}

\newenvironment{thmitemize}
{
    \leavevmode\vspace{-1.4em}
    \begin{itemize}
    }
    {
    \end{itemize}
}

% chapters = sections (otherwise numbering will not work)
\let\chapter\section

% subsections numbered by capital arabic letters
%\renewcommand{\thesubsection}{\thesection.\Roman{subsection}}
\renewcommand{\thesubsection}{\Alph{subsection})}

\usepackage{secdot}
\sectionpunct{subsection}{ }

% captions
\usepackage{capt-of}
\usepackage{caption}
\DeclareCaptionFont{white}{\color{white}}
\DeclareCaptionFormat{listing}
{
    \colorbox[cmyk]{1, 1, 1,0.01}
    {
        \parbox{\textwidth}
        {\hspace{15pt}#1#2#3}
    }
}
%\captionsetup[lstlisting]
%{
%    format=listing,
%    labelfont=white,
%    textfont=white,
%    singlelinecheck=false,
%    margin=0pt,
%    font={bf,footnotesize}
%}

% listings
\usepackage{listings}
\lstset{
    numbers=left,
    numberstyle=\tiny,
    numbersep=5pt,
    keywordstyle=\color{black}\bfseries,
    stringstyle=\ttfamily,
    showstringspaces=false,
    basicstyle=\footnotesize,
    captionpos=b
}
\lstset{language=java}
% Listings
\lstset{
    basicstyle=\fontsize{9}{9}\ttfamily, % Standardschrift
    numbers=left,               % Ort der Zeilennummern
    numberstyle=\tiny,          % Stil der Zeilennummern
    %stepnumber=2,               % Abstand zwischen den Zeilennummern
    numbersep=5pt,              % Abstand der Nummern zum Text
    tabsize=4,                  % Groesse von Tabs
    extendedchars=true,         %
    breaklines=true,            % Zeilen werden Umgebrochen
    keywordstyle=\text,
    %frame=b,         
    stringstyle=\color{black}\ttfamily, % Farbe der String
    showspaces=false,           % Leerzeichen anzeigen ?
    showtabs=false,             % Tabs anzeigen ?
    xleftmargin=5pt,
    framexleftmargin=17pt,
    framexrightmargin=5pt,
    framexbottommargin=4pt,
    %backgroundcolor=\color{lightgray},
    showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
    captionpos=t,     
}

\lstloadlanguages{% Check Dokumentation for further languages ...
    %[Visual]Basic
    %Pascal
    %C
    %C++
    %XML
    %HTML
    Java
}

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}

\newcommand{\maxpts}[1]
{
    \vspace*{-1.5cm}
    \hfill \fbox{\large #1 \pts}
    \vspace*{1cm}
}

\RequirePackage{scrpage2}
\pagestyle{scrheadings}
\clearscrheadings
\ohead{\hfill \quad \normalfont \page{} \pagemark/\pageref{LastPage}}


% multiplechoice
\newenvironment{multiplechoice}[2]{
    \begin{center}
        \begin{tabular}{lcc}
            & #1 & #2 \\
        }{
    \end{tabular}
\end{center}
\vspace{0.5cm}
}


\newcommand{\statement}[1]{
    #1	& $\Box$ & $\Box$ \\
}

% for proofs
\usepackage{bussproofs}

\newenvironment{exerciseDE}[2]
{
    \newpage
    \section{#1}
    \maxpts{#2}
    \vspace*{-0.7cm}
    
}
{
}

\newenvironment{exerciseEN}[2]
{
    \newpage
    \section{#1}
    \maxpts{#2}
    \vspace*{-0.7cm}
        
}
{
}

\newenvironment{firstpage}
{
    \thispagestyle{empty}
    \newgeometry{top=1cm, bottom=1cm}
}
{
    \pagebreak
    \restoregeometry
}



==> style/exsheet.tex <==
% ##############################
% EXERCISE SHEET SPECIFIC STUFF
% ##############################

% Festlegung Art der Zitierung - Havardmethode: Abkuerzung Autor + Jahr
\usepackage[style=alphabetic,backend=bibtex]{biblatex}

% underlining
\usepackage{ulem}

% remove all paragraph indentation
\usepackage{parskip}

% spacing between lines of text
\usepackage{setspace}

% enumerate etc
\usepackage{paralist}

% keyword index
\usepackage{makeidx}

% create keyword index
\makeindex

% abbreviation index
\usepackage[german]{nomencl}
\let\abbrev\nomenclature

% border size
\usepackage{geometry}
\geometry{left=2.2cm, right=2.2cm, top=2cm, bottom=2cm, foot= 1cm}

% Indentation
% space between lines
\onehalfspacing
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000

%  headline / footline
\usepackage{fancyhdr} %Paket laden
\pagestyle{fancy} %eigener Seitenstil

%% Seitennummer immer oben rechts
%% alle Kopf- und Fußzeilenfelder bereinigen
%\fancyhf{}
%% Kopfzeile links: Name des Kapitels = der Sektion
%\fancyhead[L]{\nouppercase{\leftmark}}
%% Kopfzeile zentriert:
%\fancyhead[C]{} 
%% Kopfzeile rechts = Seitennummer
%\fancyhead[R]{\thepage} 
%% Trennlinien
%\renewcommand{\headrulewidth}{0.4pt} 
%%\renewcommand{\footrulewidth}{0.4pt}
%% Analog
%%\fancyfoot[C]{\thepage}


% Seitennummer immer oben rechts
% alle Kopf- und Fußzeilenfelder bereinigen
\fancyhf{}
\fancyfoot[C]{}
\renewcommand{\headrule}{} 

% references
\usepackage[bookmarksnumbered]{hyperref} 

% line break in URLs
%\usepackage[hyphens,obeyspaces,spaces]{url}

% newline after paragraph, paragraph bold and underlined
\makeatletter
\renewcommand {\paragraph}
{
    \@startsection
        {paragraph} % name
        {4}         % level
        {\z@}       % indent     
        {0ex \@plus -1ex \@minus -.2ex} % beforeskip
        %{-3.25ex\@plus -1ex \@minus -.2ex} % beforeskip
        {0.01ex \@plus .2ex}                % afterskip
        %{1.5ex \@plus -2ex}                % afterskip
        {\normalfont\normalsize\bfseries\underbar} % style of heading
}
\makeatother

% proof in bold font, colon and newline afterwards
\makeatletter
\renewenvironment{proof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\\*\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother

% set emph back to normal (instead of underlined)
\normalem 

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother

% Theoremstyle
\newtheoremstyle{withnumber} % name
{0.4cm}                    % Space above
{0.6cm}                    % Space below
{\normalfont}                   % Body font
{}                           % Indent amount
{\bfseries}                   % Theorem head font
{\newline}                          % Punctuation after theorem head
{0.2cm}                       % Space after theorem head
{#1 #2\thmnote{: \ #3}}  % Theorem head spec (can be left empty, meaning ‘normal’)

\newtheoremstyle{nonumber} % name
{0.4cm}                    % Space above
{0.6cm}                    % Space below
{\normalfont}                   % Body font
{}                           % Indent amount
{\bfseries}                   % Theorem head font
{\newline}                          % Punctuation after theorem head
{0.2cm}                       % Space after theorem head
{#1\thmnote{: \ #3}}  % Theorem head spec (can be left empty, meaning ‘normal’)

\theoremstyle{withnumber} 


% itemize/enumerate at the beginning of a thm
\newenvironment{thmenumerate}
{
    \leavevmode\vspace{-1.4em}
    \begin{enumerate}
    }
    {
    \end{enumerate}
}

\newenvironment{thmitemize}
{
    \leavevmode\vspace{-1.4em}
    \begin{itemize}
    }
    {
    \end{itemize}
}

% chapters = sections (otherwise numbering will not work)
%\let\chapter\section

% subsections numbered by capital arabic letters
%\renewcommand{\thesubsection}{\thesection.\Roman{subsection}}
\renewcommand{\thesubsection}{\Alph{subsection})}

\usepackage{secdot}
\sectionpunct{subsection}{ }


% captions
\usepackage{capt-of}
\usepackage{caption}
\DeclareCaptionFont{white}{\color{white}}
\DeclareCaptionFormat{listing}
{
    \colorbox[cmyk]{1, 1, 1,0.01}
    {
        \parbox{\textwidth}
        {\hspace{15pt}#1#2#3}
    }
}
\captionsetup[lstlisting]
{
    format=listing,
    labelfont=white,
    textfont=white,
    singlelinecheck=false,
    margin=0pt,
    font={bf,footnotesize}
}

% listings
\usepackage{listings}
\lstset{
    numbers=left,
    numberstyle=\tiny,
    numbersep=5pt,
    keywordstyle=\color{black}\bfseries,
    stringstyle=\ttfamily,
    showstringspaces=false,
    basicstyle=\footnotesize,
    captionpos=b
}
\lstset{language=java}
% Listings
\lstset{
    basicstyle=\fontsize{9}{9}\ttfamily, % Standardschrift
    numbers=left,               % Ort der Zeilennummern
    numberstyle=\tiny,          % Stil der Zeilennummern
    %stepnumber=2,               % Abstand zwischen den Zeilennummern
    numbersep=5pt,              % Abstand der Nummern zum Text
    tabsize=4,                  % Groesse von Tabs
    extendedchars=true,         %
    breaklines=true,            % Zeilen werden Umgebrochen
    keywordstyle=\text,
    %frame=b,         
    stringstyle=\color{black}\ttfamily, % Farbe der String
    showspaces=false,           % Leerzeichen anzeigen ?
    showtabs=false,             % Tabs anzeigen ?
    xleftmargin=5pt,
    framexleftmargin=17pt,
    framexrightmargin=5pt,
    framexbottommargin=4pt,
    %backgroundcolor=\color{lightgray},
    showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
    captionpos=t,     
}

\lstloadlanguages{% Check Dokumentation for further languages ...
    %[Visual]Basic
    %Pascal
    %C
    %C++
    %XML
    %HTML
    Java
}

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}

\newtoks\lecturer
\newtoks\organizer
\newtoks\institution
\newtoks\term
\newtoks\releasedate
\newtoks\duedate

\makeatletter
\newcommand{\head}
{
%   \newgeometry{top=1cm}
    \vspace*{-3\baselineskip}
    %\null
    %\thispagestyle{empty}
    %\begin{center} 
    \framebox{
        \parbox{\textwidth}
        {
            \vspace*{0.2cm}
            \begin{center}
                \textrm{\textbf{\large \@title}} \\
                \textrm{\textbf{\large \@subtitle}}
            \end{center}
            \vspace*{-0.5cm}
            \begin{tabu} to \textwidth {l X r}
                \small \the\lecturer  & & \small \the\institution \\
                \small \the\organizer  & & \small \the\term \\
            \end{tabu}
        }
    } 
    %\end{center}
    %\null
    \begin{tabu} to 1.025\columnwidth {@{} l X r @{}}
        \the\releasedate  & & \the \duedate \\
    \end{tabu}
%    \vspace*{0.2cm}
%    \restoregeometry
}
\makeatother

\makeatletter
\newcommand {\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand {\problemshort}[1]{\gdef\@problemshort{#1}}% Store problem short notation
\newcommand {\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand {\problemparameter}[1]{\gdef\@problemparameter{#1}}% Store problem parameter
\newcommand {\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question

\NewEnviron{problem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocDecide:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\NewEnviron{compproblem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocCompute:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\makeatother


==> style/helvetica.tex <==
% #######
% HELVETICA
% #######

% Helvetica pro for text (and math)
% Consolas for monospace
% Euler for math

\usepackage{helvet}
\renewcommand{\familydefault}{\sfdefault}

\usepackage{isomath}
\usepackage{sansmathfonts}


==> style/ieee_additions.tex <==
% #####################
% ADDITIONS FOR LIPICS
% #####################
% some paper specific stuff

\usepackage{paralist}
\theoremstyle{plain}

\newtheorem {theorem}       {Theorem}     []
\newtheorem {corollary}		[theorem]     {Corollary}
\newtheorem {lemma}			[theorem]     {Lemma}
\newtheorem {proposition}	[theorem]     {Proposition}
\newtheorem {remark}		[theorem]     {Remark}
\newtheorem {definition}	[theorem]     {Definition}
\newtheorem {notation}		[theorem]     {Notation}
\newtheorem {example}		[theorem]     {Example}
\newtheorem {exercise}		[theorem]     {Exercise}
\newtheorem {algo}			[theorem]     {Algorithm}
\newtheorem {claim}			[theorem]     {Claim}

\sloppy
\clubpenalty = 10000 
\widowpenalty = 10000 
\displaywidowpenalty = 10000

%compact llncs-like paragraph
\newcommand{\compactparagraph}[1]{%
    \medskip%
    \noindent%
    {\bf \sffamily #1.}%
}

\newcommand{\subparagraph}[1]{%
    \medskip%
    \noindent%
    {\bf \sffamily #1.}%
}


==> style/includes.tex <==
% ##########
% INCLUDES
% ##########

% images, ...
%\usepackage{graphicx}

% tables (over several pages)
%\usepackage{array}
\usepackage{tabu}
%\usepackage{longtable}

% boxes in the text
%\usepackage{fancybox}


% see myriad.tex
\usepackage{amsmath}

% mathematic symbols
\usepackage{amssymb}
\usepackage{amssymb}
\usepackage{stmaryrd} 
\usepackage{amsthm}
\usepackage{wasysym}

% binary ops, for comparasion only
%\usepackage{shuffle} % not compatible with LIPIcs

% for coloring stuff
\usepackage{xcolor}

% for colored cells in tables
\usepackage{colortbl}

% bmatrix* with alignment
%\usepackage{mathtools}

% symbol scaling in math mode
\usepackage{scalerel}

% for symbol stacking
\usepackage{stackengine}

% \include* without new page
%\usepackage{newclude}

% parse optional arguments
\usepackage{xparse}

% subimport
%\usepackage{import}

% fix some spacing issues
\usepackage{microtype}

% floating figures
%\usepackage{wrapfig}

% custom environments
\usepackage{environ}

% ????
%\usepackage{bm}
%\usepackage{oldgerm}
%\usepackage{texdraw}
%\usepackage{multirow}





==> style/lang_de.tex <==
% ###################################
% LANGUAGE DEPENDANT STUFF: DEUTSCH
% ###################################

%
% Packages
%

\usepackage[ngerman]{babel}
\usepackage[utf8]{inputenc}
\usepackage{csquotes}

%
% Commands
%

\newcommand{\pts}{Punkte}
\newcommand{\page}{Seite}

\newcommand {\quot} [1] {\glqq #1\grqq}

\newcommand{\ProblemLocGiven}{Gegeben}
\newcommand{\ProblemLocDecide}{Entscheide}
\newcommand{\ProblemLocCompute}{Berechne}


==> style/lang_en.tex <==
% ###################################
% LANGUAGE DEPENDANT STUFF: ENGLISH
% ###################################

%
% Packages
%

%\usepackage[T1]{fontenc} % WTF!?
\usepackage[english]{babel}
\usepackage{csquotes}

%
% Commands
%

\newcommand{\pts}{points}
\newcommand{\page}{Page}

\newcommand {\quot} [1] {\enquote{#1}}

\newcommand{\ProblemLocGiven}{Given}
\newcommand{\ProblemLocDecide}{Decide}
\newcommand{\ProblemLocCompute}{Compute}



==> style/letter.tex <==
% ########################
% ARTICLE SPECIFIC STUFF
% ########################

% Festlegung Art der Zitierung - Havardmethode: Abkuerzung Autor + Jahr
\usepackage[style=alphabetic,backend=bibtex]{biblatex}

% underlining
\usepackage{ulem}

% remove all paragraph indentation
\usepackage{parskip}

% spacing between lines of text
\usepackage{setspace}

% enumerate etc
\usepackage{paralist}

% keyword index
\usepackage{makeidx}

% create keyword index
\makeindex

% abbreviation index
\usepackage[german]{nomencl}
\let\abbrev\nomenclature

% border size
\usepackage{geometry}
% top is later changed, just for title page
\geometry{left=2.5cm, right=2.5cm, top=2.5cm, bottom=2cm, foot= 1cm}

% Indentation
% space between lines
\onehalfspacing
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000

%\usepackage{scrpage2}
%\pagestyle{scrheadings}
%\cfoot{\pagemark}

%  headline / footline
\usepackage{fancyhdr} %Paket laden
\pagestyle{fancy} %eigener Seitenstil

%% Seitennummer immer oben rechts
%% alle Kopf- und Fußzeilenfelder bereinigen
%\fancyhf{}
%% Kopfzeile links: Name des Kapitels = der Sektion
%\fancyhead[L]{\nouppercase{\leftmark}}
%% Kopfzeile zentriert:
%\fancyhead[C]{} 
%% Kopfzeile rechts = Seitennummer
%\fancyhead[R]{\thepage} 
%% Trennlinien
%\renewcommand{\headrulewidth}{0.4pt} 
%%\renewcommand{\footrulewidth}{0.4pt}
%% Analog
%%\fancyfoot[C]{\thepage}


% Seitennummer immer oben rechts
% alle Kopf- und Fußzeilenfelder bereinigen
\fancyhf{}
\fancyfoot[C]{\thepage}
\renewcommand{\headrule}{} 

% references
\usepackage[bookmarksnumbered]{hyperref} 

% line break in URLs
%\usepackage[hyphens,obeyspaces,spaces]{url}

% newline after paragraph, paragraph bold and underlined
\makeatletter
\renewcommand {\paragraph}
{
    \@startsection
        {paragraph} % name
        {4}         % level
        {\z@}       % indent     
        {0ex \@plus -1ex \@minus -.2ex} % beforeskip
        %{-3.25ex\@plus -1ex \@minus -.2ex} % beforeskip
        {0.01ex \@plus .2ex}                % afterskip
        %{1.5ex \@plus -2ex}                % afterskip
        {\normalfont\normalsize\bfseries\underbar} % style of heading
}
\makeatother

% proof in bold font, colon and newline afterwards
\makeatletter
\renewenvironment{proof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\\*\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother

% set emph back to normal (instead of underlined)
\normalem 

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother

% Theorem numbering
\def\theoremnumberstyle{changesection}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Zu verwendende Regelsaetze 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Bei Nummerierung vom Typ swapped soll abweichend vom Standard
%%% "5.12. Satz" erscheinen als "5.12 Satz", das heisst ohne
%%% zusaetzlichen Punkt.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\def\swappedhead#1#2#3{%
%    \thmnumber{#2}\thmname{\@ifnotempty{#2}{ }#1}%
%    \thmnote{ {\the\thm@notefont(#3)}}}

\def\swappedhead#1#2#3{%
    \thmnumber{#2}\thmname{ #1}%
    \thmnote{ {\the\thm@notefont(#3)}}}

\newtheoremstyle{varthm-roman-break}% name
{}%      Space above, empty = `usual value'
{}%      Space below
{\normalfont}% Body font
{}%         Indent amount (empty = no indent, \parindent = para indent)
{\bfseries}% Thm head font
{}%        Punctuation after thm head
{\newline}%     Space after thm head: " " = normal interword space;
%       \newline = linebreak
{\thmnote{#3}}% Thm head spec


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Eigene Befehle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Label an beliebiger Stelle mit beliebigem Symbol setzen
% \mylabel{labelname}{(*)} liefert (*) nach \ref{labelname}
\catcode`@=11%%% Sorgt daruer, dass @ in Marconamen verwendet werden kann
\newcommand{\mylabel}[2]{\@bsphack
    \protected@write\@auxout{}%
    {\string\newlabel{#1}{{#2}{\thepage}}}%
    \@esphack}
\newcommand{\tmylabel}[2]{\@bsphack
    \protected@write\@auxout{}%
    {\string\newlabel{#1}{{#2}{\thepage}{\arabic{chapter}}}}%
    \@esphack}
\catcode`@=\active%
%%% Erzeugt an der Stelle des Aufrufs einen nicht sichtbaren Punkt.
\newcommand{\leererpunkt}{
    \drawdim pt
    \begin{texdraw}
        \setgray 1
        \lcir r:0.01       
    \end{texdraw}
}

\swapnumbers
\theoremstyle{varthm-roman-break} 

\newtheorem {theorem}	    {Theorem}     [section]
\newtheorem {corollary}		[theorem]     {Corollary}
\newtheorem {lemma}			[theorem]     {Lemma}
\newtheorem {proposition}	[theorem]     {Proposition}
\newtheorem {remark}		[theorem]     {Remark}
\newtheorem {definition}	[theorem]     {Definition}
\newtheorem {notation}		[theorem]     {Notation}
\newtheorem {example}		[theorem]     {Example}
\newtheorem {exercise}		[theorem]     {Example}
\newtheorem {algo}			[theorem]     {Algorithm}
\newtheorem {claim}			[theorem]     {Claim}

% itemize/enumerate at the beginning of a thm
\newenvironment{thmenumerate}
{
    \leavevmode\vspace{-1.4em}
    \begin{enumerate}
    }
    {
    \end{enumerate}
}

\newenvironment{thmitemize}
{
    \leavevmode\vspace{-1.4em}
    \begin{itemize}
    }
    {
    \end{itemize}
}

% chapters = sections (otherwise numbering will not work)
\let\chapter\section

% subsections numbered by capital arabic letters
%\renewcommand{\thesubsection}{\thesection.\Roman{subsection}}
\renewcommand{\thesubsection}{\Alph{subsection})}

\usepackage{secdot}
\sectionpunct{subsection}{ }


% captions
\usepackage{capt-of}
\usepackage{caption}
\DeclareCaptionFont{white}{\color{white}}
\DeclareCaptionFormat{listing}
{
    \colorbox[cmyk]{1, 1, 1,0.01}
    {
        \parbox{\textwidth}
        {\hspace{15pt}#1#2#3}
    }
}
\captionsetup[lstlisting]
{
    format=listing,
    labelfont=white,
    textfont=white,
    singlelinecheck=false,
    margin=0pt,
    font={bf,footnotesize}
}

% listings
\usepackage{listings}
\lstset{
    numbers=left,
    numberstyle=\tiny,
    numbersep=5pt,
    keywordstyle=\color{black}\bfseries,
    stringstyle=\ttfamily,
    showstringspaces=false,
    basicstyle=\footnotesize,
    captionpos=b
}
\lstset{language=java}
% Listings
\lstset{
    basicstyle=\fontsize{9}{9}\ttfamily, % Standardschrift
    numbers=left,               % Ort der Zeilennummern
    numberstyle=\tiny,          % Stil der Zeilennummern
    %stepnumber=2,               % Abstand zwischen den Zeilennummern
    numbersep=5pt,              % Abstand der Nummern zum Text
    tabsize=4,                  % Groesse von Tabs
    extendedchars=true,         %
    breaklines=true,            % Zeilen werden Umgebrochen
    keywordstyle=\text,
    %frame=b,         
    stringstyle=\color{black}\ttfamily, % Farbe der String
    showspaces=false,           % Leerzeichen anzeigen ?
    showtabs=false,             % Tabs anzeigen ?
    xleftmargin=5pt,
    framexleftmargin=17pt,
    framexrightmargin=5pt,
    framexbottommargin=4pt,
    %backgroundcolor=\color{lightgray},
    showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
    captionpos=t,     
}

\lstloadlanguages{% Check Dokumentation for further languages ...
    %[Visual]Basic
    %Pascal
    %C
    %C++
    %XML
    %HTML
    Java
}

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}


\newtoks\receiver
\newtoks\address
\newtoks\postalbox
\newtoks\plz
\newtoks\telnr
\newtoks\email

\catcode`\@ = 11 % Macro \makeatletter does the same

%\newcommand{ \at } { \makeatletter @ \makeatother }

\newcommand {\letterhead}
{
    
    \begin{tabu} to \textwidth {lXr}
        \large \the\receiver       & & \large Sebastian Muskalla\\
        \small \the\address     & & \small Institut für Theoretische Informatik\\
        \small \the\postalbox  & & \small Mühlenpfordtstr. 23\\
        \small \the\plz       & & \small 38106 Braunschweig\\
        \small \the\telnr     & & \small Tel.:  +49 (0)531 391 9520 \\
        \small \the\email     & & \small E-Mail: s.muskalla{\!\at \!}tu-bs.de\\
                                & & \\
                                & & Braunschweig, den \today \\
    \end{tabu}
    \makeatother
}

\newcommand {\lettertitle}
{\mbox{}\\\textbf{\Large{\@title}}\\}




==> style/lipics_additions.tex <==
% #####################
% ADDITIONS FOR LIPICS
% #####################
% some paper specific stuff

\usepackage{paralist}

\theoremstyle{plain}
\newtheorem {proposition} [theorem] {Proposition}
\newtheorem {claim} [theorem] {Claim}

\theoremstyle{definition}
\newtheorem {algo} [theorem] {Algorithm}
\newtheorem {rmk} [theorem] {Remark}

\sloppy
\clubpenalty = 10000 
\widowpenalty = 10000 
\displaywidowpenalty = 10000


% fake greek capitals
\newcommand {\Alpha} {A}
\newcommand {\Beta} {B}
\newcommand {\Epsilon} {E}
\newcommand {\Zeta} {Z}
\newcommand {\Eta} {H}
\newcommand {\Iota} {I}
\newcommand {\Kappa} {K}
\newcommand {\Mu} {M}
\newcommand {\Tau} {T}
\newcommand {\Chi} {X}


\newcommand {\quot} [1] {\enquote{#1}}

\newcommand{\ProblemLocGiven}{Given}
\newcommand{\ProblemLocDecide}{Decide}
\newcommand{\ProblemLocCompute}{Compute}

\makeatletter
\newcommand {\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand {\problemshort}[1]{\gdef\@problemshort{#1}}% Store problem short notation
\newcommand {\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand {\problemparameter}[1]{\gdef\@problemparameter{#1}}% Store problem parameter
\newcommand {\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question

\NewEnviron{problem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocDecide:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\NewEnviron{compproblem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocCompute:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\makeatother


==> style/misc.tex <==
% ##########
% MISC
% ##########

% Fix delimiter spacing

\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}


% Custom symbols

% triangle qed
\newcommand{\tqed}{\hfill \text{$\blacktriangleleft$}}

% item with arrow symbol like in Meyer's lectures
\newcommand {\itemarrow} 
{ {\raisebox{0.8mm}{\rotatebox[origin=c]{180}{$\Lsh$}}} } 
    
 
% Use slanted versions of leq & geq by default

% store old symbols
\let\leqstraight\leq % or just use le
\let\geqstraight\geq % or just use ge
\let\nleqstraight\nleq
\let\ngeqstraight\ngeq
\let\nle\nleq
\let\nge\ngeq

% overwrite
\let\leq\leqslant
\let\geq\geqslant
\let\nleq\leqslant
\let\ngeq\ngeqslant


==> style/myriad.tex <==
% #######
% MYRIAD
% #######

% REQUIRES XELATEX!

% Consolas and Myriad Pro have to be installed

% - upright myriad for text
% - italic myriad formath
% - consolas for monospace
% - euler for greek letters

% package to change font in XeTeX
\usepackage{mathspec}

% euler font for math
\usepackage[mathbf]{euler}
    
% default font: Myriad pro
% (has to be installed!)
\setmainfont{Myriad Pro}
\setsansfont{Myriad Pro}
\newfontfamily\myriad{Myriad Pro}

% monospace font: Consolas
% (has to be installed!)
\setmonofont{Consolas}

% use normal text font for math
\usepackage[noendash,italic]{mathastext}

% hack for emptyset
\renewcommand{\emptyset}{ {\diameter} }

% font for section, part, ... titles (in text and in table of contents)
\addtokomafont{title}{\myriad}
\setkomafont{subsection}{\bfseries\Large\myriad}
\setkomafont{section}{\bfseries\huge\myriad}
\setkomafont{sectionentry}{\bfseries\myriad} % entry in TOC
\setkomafont{part}{\bfseries\Huge\myriad} % part name
\setkomafont{partnumber}{\bfseries\Huge\myriad} % "Part II."
\setkomafont{partentry}{\bfseries\large\myriad} % entry in TOC
\setkomafont{paragraph}{\bfseries\myriad}
\setkomafont{subparagraph}{\bfseries\myriad} % entry in TOC

% Take nice sans-serif greek letters from the font "Euler"
%\DeclareSymbolFont{EulerGreek}{U}{eur}{m}{n}
%\DeclareMathSymbol\Gamma    {\mathalpha}{EulerGreek}{"00}
%\DeclareMathSymbol\Delta    {\mathalpha}{EulerGreek}{"01}
%\DeclareMathSymbol\Theta    {\mathalpha}{EulerGreek}{"02}
%\DeclareMathSymbol\Lambda   {\mathalpha}{EulerGreek}{"03}
%\DeclareMathSymbol\Xi       {\mathalpha}{EulerGreek}{"04}
%\DeclareMathSymbol\Pi       {\mathalpha}{EulerGreek}{"05}
%\DeclareMathSymbol\Sigma    {\mathalpha}{EulerGreek}{"06}
%\DeclareMathSymbol\Upsilon  {\mathalpha}{EulerGreek}{"07}
%\DeclareMathSymbol\Phi      {\mathalpha}{EulerGreek}{"08}
%\DeclareMathSymbol\Psi      {\mathalpha}{EulerGreek}{"09}
%\DeclareMathSymbol\Omega    {\mathalpha}{EulerGreek}{"0A}
%\DeclareMathSymbol{\alpha}  {\mathalpha}{EulerGreek}{"0B}
%\DeclareMathSymbol{\beta}   {\mathalpha}{EulerGreek}{"0C}
%\DeclareMathSymbol{\gamma}  {\mathalpha}{EulerGreek}{"0D}
%\DeclareMathSymbol{\delta}  {\mathalpha}{EulerGreek}{"0E}
%\DeclareMathSymbol{\epsilon}{\mathalpha}{EulerGreek}{"0F}
%\DeclareMathSymbol{\zeta}   {\mathalpha}{EulerGreek}{"10}
%\DeclareMathSymbol{\eta}    {\mathalpha}{EulerGreek}{"11}
%\DeclareMathSymbol{\theta}  {\mathalpha}{EulerGreek}{"12}
%\DeclareMathSymbol{\iota}   {\mathalpha}{EulerGreek}{"13}
%\DeclareMathSymbol{\kappa}  {\mathalpha}{EulerGreek}{"14}
%\DeclareMathSymbol{\lambda} {\mathalpha}{EulerGreek}{"15}
%\DeclareMathSymbol{\mu}     {\mathalpha}{EulerGreek}{"16}
%\DeclareMathSymbol{\nu}     {\mathalpha}{EulerGreek}{"17}
%\DeclareMathSymbol{\xi}     {\mathalpha}{EulerGreek}{"18}
%\DeclareMathSymbol{\pi}     {\mathalpha}{EulerGreek}{"19}
%\DeclareMathSymbol{\rho}    {\mathalpha}{EulerGreek}{"1A}
%\DeclareMathSymbol{\sigma}  {\mathalpha}{EulerGreek}{"1B}
%\DeclareMathSymbol{\tau}    {\mathalpha}{EulerGreek}{"1C}
%\DeclareMathSymbol{\upsilon}{\mathalpha}{EulerGreek}{"1D}
%\DeclareMathSymbol{\phi}    {\mathalpha}{EulerGreek}{"1E}
%\DeclareMathSymbol{\chi}    {\mathalpha}{EulerGreek}{"1F}
%\DeclareMathSymbol{\psi}    {\mathalpha}{EulerGreek}{"20}
%\DeclareMathSymbol{\omega}  {\mathalpha}{EulerGreek}{"21}
%\DeclareMathSymbol{\varepsilon}{\mathalpha}{EulerGreek}{"22}
%\DeclareMathSymbol{\vartheta}{\mathalpha}{EulerGreek}{"23}
%\DeclareMathSymbol{\varpi}  {\mathalpha}{EulerGreek}{"24}
%\DeclareMathSymbol{\varphi} {\mathalpha}{EulerGreek}{"27}
%\DeclareMathSymbol\upOmega  {\mathord}{EulerGreek}{"0A}
%\DeclareMathSymbol\upDelta  {\mathord}{EulerGreek}{"01}

% blackbord bold letters
%\DeclareMathAlphabet{\mathds}{U}{dsrom}{m}{n}
\usepackage[bb=fourier]{mathalfa}


==> style/nth.tex <==
% nth.sty  version 2002/27/02 Donald Arseneau
% Ordinal numbering style, 1st 2nd 3rd 4th 5th... 12th... 101st 102nd...
%
% (Public domain: take, include, extract, whatever)
%
% In LaTeX: 
%           \usepackage[super,negative]{nth}
% where option [super] gives superscript `th'
% and option [negative] allows ``st, nd, rd'' suffixes on negative numbers.
%
% example:  \renewcommand{\thesection}{\ordinal{section}}
% or        \renewcommand{\thesection}{\@ordinal\c@section}
% or        \renewcommand{\thesection}{\nth\c@section}
%   
% In plain TeX: 
%           \input nth.sty
% use:      \nth{<number>}.
% Change formatting by redefining \nthscript and \nthtest

% modified to be also able to do things like \nth{i}
% (in this case, always "th" is used)

% ToDo:
% \nth{(n+1)} should give (n+1)^st

\usepackage{xstring}

\def\nth#1{
    \IfInteger{#1}
    {\nthH{#1}}
    {#1\nthscript{th}}
}

\def\nthH#1{% First print number:
    \expandafter\nthM \number #1\relax
    \nthscript{%
        \ifnum#1\nthtest0 th\else % negatives are all ``th'' (depending on \nthtest)
        \expandafter \nthSuff \expandafter 0\number\ifnum #1<0-\fi#1\delimiter
        \fi
    }}
    
% Minus sign using math mode:
\def\nthM#1{\if -#1\ifmmode-\else$-$\fi\else #1\fi}

% Print suffix depending on last two digits:
\def\nthSuff#1#2#3{%
    \ifx \delimiter#3% #1#2 are last two digits
    \ifnum #1=1 th%  teens are always ``th''
    \else % use appropriate suffix
    \ifcase #2 th\or st\or nd\or rd\else th\fi
    \fi
    \else % continue scanning for last two digits
    \expandafter \nthSuff \expandafter #2\expandafter #3%
    \fi}

% Formatting hook for ordinals (\let\nthscript\textsuperscript)
\def\nthscript#1{\textsuperscript{#1}}% alternate: \def\nthscript#1{$\rm^{#1}$}

% Formatting hook for all negative numbers giving ``th''
\def\nthtest{=}  % alternate: \def\nthtest{=}

%\ifx\Alph\undefined\else
%\def\ordinal#1{\expandafter\@ordinal\csname c@#1\endcsname}
%\let\@ordinal\nth
%\ProvidesPackage{smnth}[2016/05/31] % yyyy-mm-dd
%\DeclareOption{super}{\def\nthscript#1{#1}}
%\DeclareOption{negative}{\def\nthtest{<}}
%\ProcessOptions
%\fi
%    


==> style/operators.tex <==
% ##################
% OPERATORS
% ##################

%\DeclareMathOperator{\Attr}{Attr}
\DeclareMathOperator{\bin}{bin}


==> style/presentation.tex <==
% #######################
% BEAMER SPECIFIC STUFF
% #######################

% Metropolis theme
% (has to be installed)
\usetheme{metropolis}

% ???
\usepackage{booktabs}
\usepackage[scale=2]{ccicons}

% stuff for tikz
\usepackage{pgfplots}
\usepgfplotslibrary{dateplot}

% absolute positioning of boxes
\usepackage[absolute,overlay]{textpos}

% enumeration
\usepackage{enumerate}

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}



==> style/stix.tex <==
% #######
% STIX
% #######


% - myriad for text and math
% - consolas for monospace
% - euler for greek letters

% REQUIRES XELATEX!

% Consolas and Myriad Pro have to be installed

% Myriad pro for text (and math)
% Consolas for monospace
% Euler for math

\usepackage[notext]{stix}

% package to change font in XeTeX
\usepackage[no-math]{fontspec}

% euler font for math
%\usepackage[mathbf]{euler}
    
% default font: Myriad pro
% (has to be installed!)
\setmainfont{Myriad Pro}
\setsansfont{Myriad Pro}
\newfontfamily\myriad{Myriad Pro}

% monospace font: Consolas
% (has to be installed!)
\setmonofont{Consolas}

% use normal text font for math
%\usepackage[noendash,italic]{mathastext}

% hack for emptyset
\renewcommand{\emptyset}{ {\diameter} }

% font for section, part, ... titles (in text and in table of contents)
\usepackage{titlesec}
\addtokomafont{title}{\myriad}
\setkomafont{subsection}{\bfseries\Large\myriad}
\setkomafont{section}{\bfseries\huge\myriad}
\setkomafont{sectionentry}{\bfseries\myriad} % entry in TOC
\setkomafont{part}{\bfseries\Huge\myriad} % part name
\setkomafont{partnumber}{\bfseries\Huge\myriad} % "Part II."
\setkomafont{partentry}{\bfseries\large\myriad} % entry in TOC
\setkomafont{paragraph}{\bfseries\myriad}
\setkomafont{subparagraph}{\bfseries\myriad} % entry in TOC

% Take nice sans-serif greek letters from the font "Euler"
%\DeclareSymbolFont{EulerGreek}{U}{eur}{m}{n}
%\DeclareMathSymbol\Gamma    {\mathalpha}{EulerGreek}{"00}
%\DeclareMathSymbol\Delta    {\mathalpha}{EulerGreek}{"01}
%\DeclareMathSymbol\Theta    {\mathalpha}{EulerGreek}{"02}
%\DeclareMathSymbol\Lambda   {\mathalpha}{EulerGreek}{"03}
%\DeclareMathSymbol\Xi       {\mathalpha}{EulerGreek}{"04}
%\DeclareMathSymbol\Pi       {\mathalpha}{EulerGreek}{"05}
%\DeclareMathSymbol\Sigma    {\mathalpha}{EulerGreek}{"06}
%\DeclareMathSymbol\Upsilon  {\mathalpha}{EulerGreek}{"07}
%\DeclareMathSymbol\Phi      {\mathalpha}{EulerGreek}{"08}
%\DeclareMathSymbol\Psi      {\mathalpha}{EulerGreek}{"09}
%\DeclareMathSymbol\Omega    {\mathalpha}{EulerGreek}{"0A}
%\DeclareMathSymbol{\alpha}  {\mathalpha}{EulerGreek}{"0B}
%\DeclareMathSymbol{\beta}   {\mathalpha}{EulerGreek}{"0C}
%\DeclareMathSymbol{\gamma}  {\mathalpha}{EulerGreek}{"0D}
%\DeclareMathSymbol{\delta}  {\mathalpha}{EulerGreek}{"0E}
%\DeclareMathSymbol{\epsilon}{\mathalpha}{EulerGreek}{"0F}
%\DeclareMathSymbol{\zeta}   {\mathalpha}{EulerGreek}{"10}
%\DeclareMathSymbol{\eta}    {\mathalpha}{EulerGreek}{"11}
%\DeclareMathSymbol{\theta}  {\mathalpha}{EulerGreek}{"12}
%\DeclareMathSymbol{\iota}   {\mathalpha}{EulerGreek}{"13}
%\DeclareMathSymbol{\kappa}  {\mathalpha}{EulerGreek}{"14}
%\DeclareMathSymbol{\lambda} {\mathalpha}{EulerGreek}{"15}
%\DeclareMathSymbol{\mu}     {\mathalpha}{EulerGreek}{"16}
%\DeclareMathSymbol{\nu}     {\mathalpha}{EulerGreek}{"17}
%\DeclareMathSymbol{\xi}     {\mathalpha}{EulerGreek}{"18}
%\DeclareMathSymbol{\pi}     {\mathalpha}{EulerGreek}{"19}
%\DeclareMathSymbol{\rho}    {\mathalpha}{EulerGreek}{"1A}
%\DeclareMathSymbol{\sigma}  {\mathalpha}{EulerGreek}{"1B}
%\DeclareMathSymbol{\tau}    {\mathalpha}{EulerGreek}{"1C}
%\DeclareMathSymbol{\upsilon}{\mathalpha}{EulerGreek}{"1D}
%\DeclareMathSymbol{\phi}    {\mathalpha}{EulerGreek}{"1E}
%\DeclareMathSymbol{\chi}    {\mathalpha}{EulerGreek}{"1F}
%\DeclareMathSymbol{\psi}    {\mathalpha}{EulerGreek}{"20}
%\DeclareMathSymbol{\omega}  {\mathalpha}{EulerGreek}{"21}
%\DeclareMathSymbol{\varepsilon}{\mathalpha}{EulerGreek}{"22}
%\DeclareMathSymbol{\vartheta}{\mathalpha}{EulerGreek}{"23}
%\DeclareMathSymbol{\varpi}  {\mathalpha}{EulerGreek}{"24}
%\DeclareMathSymbol{\varphi} {\mathalpha}{EulerGreek}{"27}
%\DeclareMathSymbol\upOmega  {\mathord}{EulerGreek}{"0A}
%\DeclareMathSymbol\upDelta  {\mathord}{EulerGreek}{"01}

% blackbord bold letters
%\DeclareMathAlphabet{\mathds}{U}{dsrom}{m}{n}
\usepackage[bb=fourier]{mathalfa}


==> style/theorems_de.tex <==
% ######################
% THEOREM ENVIRONMENTS
% ######################

%\newtheorem {theorem}		[theorem]     {Theorem}
\newtheorem {corollary}		[theorem]     {Korollar}
\newtheorem {lemma}			[theorem]     {Lemma}
\newtheorem {proposition}	[theorem]     {Proposition}
\newtheorem {remark}		[theorem]     {Bemerkung}
\newtheorem {definition}	[theorem]     {Definition}
\newtheorem {notation}		[theorem]     {Notation}
\newtheorem {example}		[theorem]     {Beispiel}
\newtheorem {exercise}		[theorem]     {Aufgabe}
\newtheorem {algo}			[theorem]     {Algorithmus}
\newtheorem {claim}			[theorem]     {Behauptung}
\newtheorem {conjecture}	[theorem]     {Vermutung}
\newtheorem {sources}	[theorem]         {Quellen}

\theoremstyle{nonumber} 

\newtheorem* {theorem*}         {Theorem}
\newtheorem* {corollary*}       {Korollar}
\newtheorem* {lemma*}           {Lemma}
\newtheorem* {proposition*}     {Proposition}
\newtheorem* {remark*}          {Bemerkung}
\newtheorem* {definition*}      {Definition}
\newtheorem* {notation*}        {Notation}
\newtheorem* {example*}         {Beispiel}
\newtheorem* {exercise*}        {Aufgabe}
\newtheorem* {algo*}            {Algorithmus}
\newtheorem* {claim*}           {Behauptung}
\newtheorem* {conjecture*}      {Vermutung}
\newtheorem* {sources*}	        {Quellen}

\theoremstyle{numberfirst} 


==> style/theorems_en.tex <==
% ######################
% THEOREM ENVIRONMENTS
% ######################

%\newtheorem {theorem}		[theorem]     {Theorem}
\newtheorem {corollary}		[theorem]     {Corollary}
\newtheorem {lemma}			[theorem]     {Lemma}
\newtheorem {proposition}	[theorem]     {Proposition}
\newtheorem {remark}		[theorem]     {Remark}
\newtheorem {definition}	[theorem]     {Definition}
\newtheorem {notation}		[theorem]     {Notation}
\newtheorem {example}		[theorem]     {Example}
\newtheorem {exercise}		[theorem]     {Exercise}
\newtheorem {algo}			[theorem]     {Algorithm}
\newtheorem {claim}			[theorem]     {Claim}
\newtheorem {conjecture}	[theorem]     {Conjecture}
\newtheorem {sources}	    [theorem]     {Sources}

\theoremstyle{nonumber} 

\newtheorem* {theorem*}         {Theorem}
\newtheorem* {corollary*}       {Corollary}
\newtheorem* {lemma*}           {Lemma}
\newtheorem* {proposition*}     {Proposition}
\newtheorem* {remark*}          {Remark}
\newtheorem* {definition*}      {Definition}
\newtheorem* {notation*}        {Notation}
\newtheorem* {example*}         {Example}
\newtheorem* {exercise*}        {Exercise}
\newtheorem* {algo*}            {Algorithm}
\newtheorem* {claim*}           {Claim}
\newtheorem* {conjecture*}      {Conjecture}
\newtheorem* {sources*}	        {Sources}

\theoremstyle{withnumber} 


==> style/tikz.tex <==
% ########################
% TIKZ
% ########################

% Includes
\usepackage{tikz}
\usepackage{pgf}
\usetikzlibrary{arrows}
\usetikzlibrary{automata}
\usetikzlibrary{shapes}
\usetikzlibrary{backgrounds}
\usetikzlibrary{petri}
\usetikzlibrary{calc} 
\usetikzlibrary{decorations}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{positioning}
\usetikzlibrary{patterns}
\usetikzlibrary{fit}
\usetikzlibrary{graphs}
\usetikzlibrary{babel}


\tikzset{
%    treenode/.style = {align=center, inner sep=0pt, text centered,
%        font=\sffamily},
%    arn_n/.style = {treenode, circle, white, font=\sffamily\bfseries, draw=black,
%        fill=black, text width=1.5em},% arbre rouge noir, noeud noir
%    arn_r/.style = {treenode, circle, red, draw=red, 
%        text width=1.5em, very thick},% arbre rouge noir, noeud rouge
%    arn_x/.style = {treenode, rectangle, draw=black,
%        minimum width=0.5em, minimum height=0.5em},% arbre rouge noir, nil
    roundpos/.style = {treenode, circle, black, draw=black,
        minimum size=2.5em},
    squarepos/.style = {treenode, rectangle, black, draw=black,
        minimum width=2em, minimum height=2em},
}

\tikzset{
    invisible/.style={opacity=0},
    visible on/.style={alt={#1{}{invisible}}},
    alt/.code args={<#1>#2#3}{%
        \alt<#1>{\pgfkeysalso{#2}}{\pgfkeysalso{#3}} % \pgfkeysalso doesn't change the path
    },
}

\tikzset
{
    tboxoutline/.style = 
    {
        draw,
        thick,
        minimum size=6em,
        inner sep=0pt,
        outer sep=0pt,
    },
    tboxstate/.style =
    {
        minimum width=4pt,
        minimum height=2pt,
        inner sep=0pt,
        fill
    },
    tboxarrow/.style =
    {
    },
    pics/tbox/.style 2 args =
    {
        code =
        {
            \node[tboxoutline,pic actions] (-box) {};
            \foreach \i in {1,...,#1}
            {
                \path
                    (-box.north west)
                    --
                    node
                        [tboxstate,anchor=east,pos=-1/#1/2+\i/#1,pic actions]
                        (-box-in-\i)
                        {}
                    (-box.south west);
                \path
                    (-box.north east) --
                    node
                        [tboxstate,anchor=west,pos=-1/#1/2+\i/#1,pic actions]
                        (-box-out-\i)
                        {}
                (-box.south east);
            }
            
            \foreach \i/\j/\d in {#2}
            {
                \draw
                    [   
                        tboxarrow,
                        decoration =
                        {
                            markings,
                            mark=
                                at position 1 with
                                {
                                    \arrow[scale=1,>=triangle 45]{>}
                                }
                        }
                        ,
                        postaction={decorate}
                    ]
                    (-box-in-\i.east)
                    --
                    node
                        [pos=.8,\d]
                        {}
                    (-box-out-\j.west);
            }
        }
    },
    tbox color/.style={
        tboxstate/.append style={fill=#1},
        tboxoutline/.append style={draw=#1},
        tboxarrow/.append style={draw=#1},
    },
    trans/.style =
    {
        thick,
    },
    dot/.style =
    {
        circle,
        draw,
        minimum size=6pt,
        inner sep=0pt,
        fill,
    },
}

%\tikzset{
%%    place/.style = {
%%        circle,
%%        draw=blue!50,
%%        fill=blue!20,
%%        thick
%%    },
%%    bend angle = 45,
%    pre/.style = {
%        <-,
%        >= stealth',
%        semithick
%    },
%    post/.style = {
%        ->,
%        >= stealth',
%        semithick
%    },
%    recstate/.style = {
%        shape=rectangle,
%        draw,
%        rounded corners
%    },
%%    end/.style = {
%%        double
%%    },
%%    node distance = 1.6cm,
%%    gewellt/.style = {
%%        ->,
%%        line join=round,
%%        decorate, decoration={
%%            zigzag,
%%            segment length=4,
%%            amplitude=.9,post=lineto,
%%            post length=2pt
%%        }
%%    }
%}

